Transfer Learning in Human Activity Recognition: A Survey

Sensor-based human activity recognition (HAR) has been an active research area, owing to its applications in smart environments, assisted living, fitness, healthcare, etc. Recently, deep learning based end-to-end training has resulted in state-of-the-art performance in domains such as computer vision and natural language, where large amounts of annotated data are available. However, large quantities of annotated data are not available for sensor-based HAR. Moreover, the real-world settings on which the HAR is performed differ in terms of sensor modalities, classification tasks, and target users. To address this problem, transfer learning has been employed extensively. In this survey, we focus on these transfer learning methods in the application domains of smart home and wearables-based HAR. In particular, we provide a problem-solution perspective by categorizing and presenting the works in terms of their contributions and the challenges they address. We also present an updated view of the state-of-the-art for both application domains. Based on our analysis of 205 papers, we highlight the gaps in the literature and provide a roadmap for addressing them. This survey provides a reference to the HAR community, by summarizing the existing works and providing a promising research agenda.

==> acknowledgements.tex <==
This work was partially supported by CISCO.
% Add later: through grant XXX. \thomas{Ask Hugo for correct language to use here.}

==> applications.tex <==
In this section, we briefly summarize the prominent transfer learning works done in three commonplace applications domains. \thomas{So, given our specific target on sensor-based HAR -- why would we only "briefly summarize" here. This is *the* value added by this survey! The previous section is -- necessarily -- superficial because we are not writing a tutorial but a survey *on transfer learning for [sensor-based] HAR. As such, this survey can be brief on the previous section but has to be comprehensive on this one here. Otherwise, it is of little value because one could not be sure if the survey actually covers the current SOTA. To make this clear (again): This section has to be the heart of our survey!}
Here, we classify the works from a solution perspective, i.e., in terms of instance/feature/parameter transfer and present them such that a unified theme of the solution space for each domain can be understood. 

\thomas{I had mentioned that before: Somewhere in this survey we need to work out why our domain (sensor-based HAR) is so special -- I suggest early on (see my comments there). We may want to introduce a list of "special circumstances" and "problems / challenges", which we can then use to structure the applications here such that there is actual value for the community other than us just listing most recent papers in our field.}

\subsection{Activities of Daily Living using Wearables}

\begin{figure}[]
  \centering
  \includegraphics[width=\linewidth]{Figures/wearable_map.png}
  \caption{Map of the works in the ADL application domain. Here, the x-axis represents the year of publication and the y-axis represents the number of citations. Each connection represents a reference between the two works. \thomas{Again not referenced anywhere in the text. Also: Are we allowed to use that figure -- how would we reference Litmaps?}}
  %\Description{}
  \label{fig:map_wearable}
\end{figure}

Recognizing activities of daily living using wearable sensors is the most explored application domain, when it comes to transfer learning. 
A number of datasets have been collected using wearable smart devices \cite{stisen2015smart, reiss2012introducing} and smartphones \cite{chatzaki2017human} that contain Inertial Measurement Units (IMU), i.e., movement sensors. 
These IMU units \thomas{What do you think does the "U" stand for in IMUW?} consist of accelerometer, gyroscope, and magnetometer sensors that collect data corresponding to human kinematics (acceleration and angular velocity) and magnetic field. 
These units are attached on-body, for example, at  wrist, waist, chest, and ankle to sense key movement patterns that help recognize daily living activities. 
Although this application domain has advantages like the existence of large-scale annotated datasets and consistency in the sensor type \thomas{Joking, right? Read your own paper, and then read the other ones from our lab: Our *whole* work is based on the premise that there is NOT enough annotated training data. What are you talking about?} , there are still many transfer learning challenges that need to be addressed. 

Firstly, the transfer can happen between different subjects that have their idiosyncrasies embedded into the sensed data. 
Thus, cross-subject \cite{crossperson_deng_2014} activity recognition needs to be performed to mitigate the effect of subject-specific data characteristics on target performance. 
Secondly, the transfer between sensing positions \cite{crossposition_chen_2019} can take place, e.g. from wrist to chest. 
Thus, cross-position transfer learning is also a relevant research direction, where knowledge from one view is transferred to another view. 
Apart from subjects and sensing positions, there can also be changes in the sensing device and its frequency, which also needs to be incorporated into the transfer learning problem \cite{crossmobile_zhao_2010}. 
Finally, there can be special usecase-specific requirements like privacy preservation \cite{semisupervised_hashemian_2021}, distributed computations \cite{federated_gudur_2020}, real-time inference \cite{kurz2011real}, etc. 
Thus, challenges like the installation of transfer learning frameworks in federated learning, distributed environments, and online/streaming setups are also relevant.  
To address the aforesaid \thomas{Nobody uses this word ("aforesaid") ... Use "aforementioned" if you have to.} challenges, several instance, feature, and parameter-based transfer learning methods are proposed in the literature.
\thomas{So, these last two paragraphs are essentially going in the direction of what we will need to justify this survey: explaining (coarsely here) the challenges and specifics of our domain. A bit late here.}

\subsubsection{Instance-transfer}
Among the instance-based transfer learning solutions, the commonly explored methodologies are label propagation, source domain selection, boosting techniques, instance weighing, source-target data mapping, synthetic data generation, and data augmentation. 
In label propagation, the overall aim is to learn a mapping between source and target label sets using target as well as source data instances. 
An intuitive way of performing this is by initially clustering the data instances or their representations and then calculating different metrics on them for propagation \cite{plugnlearn_rokni_2016}.
These metrics include distance and similarity measurements such as centroid vector distance \cite{collaborative_kong_2020}, Wasserstein distance \cite{recurrenthar_kumar_2022}, cosine similarity \cite{evaluating_wijekoon_2020}, and RBF kernel-based similarity \cite{personalized_bettini_2021}.
Another alternative is to pose the propagation problem as graph matching \cite{autonomous_rokni_2018}. 
Here, the data instances are initially clustered to form instance communities, and then a matching problem is constructed by visualizing the communities as a bipartite or a dependency graph. 
This problem can be solved using techniques like min-cost mapping \cite{alinia2020actilabel} or weighted graph matching \cite{autonomous_rokni_2018}. 
Similarity graphs \cite{synchronous_rokni_2017} are also explored in the literature under this problem formulation. 
The problem of label propagation can also be solved without explicitly learning a mapping function by constructing a nearest class-center classifier trained on source instances \cite{adarc_roggen_2013}. 
\thomas{I thought this section is about application domains? Now we are listing techniques again?}

Next, the source domain selection approach to instance-based transfer focuses on selecting the \textit{ideal} source instances/domains for the given target domain. 
The common ways of performing source domain selection are through using distance measurements like generic, semantic, and kinetic domain distances \cite{deep_wang_2018}, stratified domain distance \cite{crossposition_chen_2019}, global and sub-domain distances \cite{dmstl_zhu_2023}, and XHAR distance \cite{xhar_zhou_2020}. 
In addition to selecting domains as a whole, there have also been works that perform relevant feature selection using perplexity scores \cite{chakma2021activity}.
Other approaches to source domain selection include learning a gating function based on the target context \cite{sharenlearn_rokni_2019} and incorporating a Bayesian optimization strategy \cite{transfer_shen_2023}. 
Finally, the source domain selection problem is also viewed as a decoupled domain variance problem \cite{vma_hu_2022}, where instead of directly transferring from the intended source to target domains, a path of intermediate domain transfers is learned, which minimizes the variation in each intermediate pair of source-target domains. 

Now \thomas{Not a talk ...}, the traditional way of performing instance transfer is via techniques like bagging, boosting, and instance weighing. 
For bagging and boosting, methods like online bagging using random forests \cite{online_sztyler_2017} and AdaBoost \cite{framework_wen_2017}, AdaBoost with LDA \cite{learning_wen_2017}, and similarity-sensitive boosting \cite{enabling_lane_2011} have been explored, respectively.
In the case of instance weighing, the weights are assigned either based on the similarity of data instances or the extent of misclassification. 
For calculating similarity, measures like mutual information \cite{towards_li_2022}, weighted MMD \cite{feature_chen_2021}, $L_{2,1}$ norm \cite{feature_chen_2021}, and log-likelihood function \cite{importanceweighted_hachiya_2012} could be used. 
Also, algorithms like kernel mean matching \cite{transfer_li_2022} and nearest neighbor weighing \cite{unsupervised_barbosa_2018} have also been used to implicitly measure this similarity. 
Finally, instance weighting schemes based on the extent of misclassification are explored using a combination of classification \cite{swladapt_hu_2023}, domain discrimination \cite{endtoend_ye_2021}, and meta-classification loss \cite{swladapt_hu_2023}, and with hierarchical Bayesian models as classifiers \cite{active_diethe_2016}.  

A more direct way of using source instances in target domain training is to learn a mapping function between the data instances. 
This mapping function can also exist between data clusters or motifs \cite{signallevel_saeedi_2020}, which are relatively more easy to map, owing to algorithms like optimal transport \cite{crossdomain_lu_2021}.   
Such mapping is often based on metrics like cosine similarity (between data points) \cite{evaluating_wijekoon_2020} and MMD measure (between clusters) \cite{local_zhao_2021}. 
A more constrained, such as linear mapping, can also be learned using QR factorization \cite{opportunistic_banos_2021}.
An extension of this mapping idea is the generation of synthetic target data by leveraging models learned from source instances. 
Many times, different data sources (modalities) are leveraged in this process, such as skeletal maps \cite{novel_fan_2022} and motion capture data \cite{learning_xia_2021}, thereby using the pre-trained models or architectures in the framework. 
More recently, GANs have also been used successfully to perform this task, based on confusion maximization \cite{systematic_chang_2020} and micro-mini batch strategy \cite{generic_soleimani_2022}. 
An indirect way of generating synthetic target instances is via data augmentations. 
In addition to the basic data transformations \cite{systematic_chang_2020}, the literature also consists of works that aim at attribute-specific and semantically aware augmentation techniques to follow domain constraints \cite{semanticdiscriminative_lu_2022}.  

\thomas{This entire (!) subsection does not mention a single application. A bit odd, given that this is the application section, don't you think?}
\subsubsection{Feature-transfer}
Feature-based transfer methods aim at projecting data instances from source and target domains onto a single representation space. 
This can either be done by learning a source-to-target feature map or by constructing an intermediate feature space. 
Literature consists of several algorithms to perform this transfer, including PCA \cite{achieving_lago_2020}, LDA \cite{framework_wen_2017}, cluster-and-match \cite{personalization_fallahzadeh_2017}, feature agglomeration \cite{additional_lago_2021}, transfer component analysis (TCA) \cite{unsupervised_barbosa_2018}, subspace alignment (SA) \cite{unsupervised_barbosa_2018}, locally linear embedding \cite{personalized_saeedi_2018}, correlation alignment (CORAL) \cite{transfer_li_2022}, and sparse coding \cite{bhattacharya2014using}.  
Both PCA and LDA can be viewed as dimensionality reduction methods while preserving inter-class differences. 
Cluster-and-match on the other hand, forms clusters of data points, communities, or views of data points, and the formed clusters are considered as the projected feature space. 
In feature agglomeration, features that are similar are clustered and merged iteratively to arrive at a common subspace. 
Next, TCA uses the MMD measure to learn transfer components in a reproducing kernel Hilbert space, whereas, in SA, the subspaces formed by top-$k$ eigenvectors of source and target domains are used to learn a mapping. 
Locally linear embedding preserves the non-linear feature structure by learning an approximation of each data instance as a linear combination of its local $k$-neighborhood. 
While these methods attempt to learn an intermediate feature space, CORAL aims at transferring the source feature space to the target using covariance matrices of the domains. 
Finally, we arrive at sparse coding, which differs from all the previous methods as it learns an over-complete set of feature vectors rather than reducing the dimensionality. 

In addition to these contributions using standard feature transfer algorithms, many works pose this problem in non-standard forms. 
For example, feature transfer is also viewed as a matrix factorization \cite{instilling_wei_2016} and a dependency graph mapping \cite{modelagnostic_alinia_2023} problem in the literature. 
In some cases, rather than learning the intermediate feature space from provided features, it is learned by using sensor \& activity context models \cite{adaptive_wen_2016}, selection of best-performing features \cite{crosslocation_janko_2019}, semantic space representation \cite{nuactiv_cheng_2013}, and semantic attribute sequence modeling \cite{towards_cheng_2013}. 


Recently, deep neural networks have been explored to perform feature mapping, where the extracted representations of source and target instances are mapped onto a common space, on which, the distributions are trained to align. 
Different architectural components like fully connected \cite{untran_khan_2018}, convolutional \cite{transfer_an_2020}, recurrent \cite{xhar_zhou_2020}, and attention \cite{tasked_suh_2022} layers are incorporated in model architecture. 
In such frameworks, the optimization problem for aligning features is posed by using losses like MMD \cite{tasked_suh_2022} and JSD \cite{augtoact_faridee_2019} loss. 
Discriminative models like bidirectional GANs can also be seen as performing feature transfer \cite{contrasgan_sanabria_2021}. 

\thomas{As before: This is a mere listing of techniques with no actual connection to let alone explanation of application domains.}

\subsubsection{Parameter-transfer}
The most common parameter-transfer paradigm that we observe \thomas{Nope ...} is pretrain-then-finetune, where a model is first pre-trained on the source domain in (un/semi/self)-supervised manner. \thomas{Repetition to the methods section.}
Then, a subset of this model is frozen and transferred to the target domain to perform finetuning on the target domain.
Architectures like AE \cite{untran_khan_2018}, VAE \cite{towards_li_2022}, CNN \cite{transfer_pavliuk_2023} (ResNet \cite{crossdataset_gjoreski_2019}, Bayesian CNN with stochastic latent variable \cite{personalizing_akbari_2020}), GRU \cite{recurrenthar_kumar_2022}, LSTM \cite{digging_hoelzemann_2020}, Bi-GAN \cite{contrasgan_sanabria_2021}, graph neural nets \cite{deep_yan_2022}, CRF \cite{remember_blanke_2010}, spatial transformer \cite{strangan_faridee_2021}, etc.\ have been tested in the literature to perform pre-training.
There are several ways in which this pre-training can be performed. \thomas{Go back to the subsection on parameter transfer in section 3 and see how repetitive this all is.}

In the case of supervised pre-training, there have been works that perform multi-source pre-training in a leave-one-dataset-out manner \cite{combining_presotto_2023}. 
Some works generate different supervised tasks by combining source domains in pre-training, which can also be carried out using meta-learning \cite{metasense_gong_2019}.
\thomas{This could be written for any application domain. Nothing specific to our focus.}

There have also been cases where different data modalities, such as pose and virtual IMU data, are used in pre-training \cite{deep_xiao_2020}. 
Moreover, vision-based models are also used, where methods like activity image creation and continuous wavelet transform are engineered to accommodate such models for IMU data \cite{transfer_pavliuk_2023}.

In some cases, these models are used separately and their predictions are forwarded to assist the base model predictions on IMU data \cite{vision_radu_2019}.    
For performing un/self-supervised pre-training, strategies like sensor modality classification \cite{deep_li_2020}, task classification \cite{domain_wilson_2022}, sensor context detection \cite{autonomous_rokni_2016}, incremental learning based on context data \cite{less_hu_2016}, pretext tasks \cite{haresamudram2022assessing} (AE, SimCLR, CPC, multi-task transformation prediction, etc.), and contrastive learning \cite{haresamudram2021contrastive} are explored. 
Pre-training can also be aimed at learning specific types of features, which is evidenced by works that target stochastic feature learning \cite{transferring_akbari_2019}, feature alignment \cite{augtoact_faridee_2019}, and disentangled feature learning. 
Among these, feature disentanglement is explored more in recent literature using mutual information based \cite{learning_xia_2021}, VAE-based \cite{latent_qian_2021}, and ELBO strategy \cite{towards_li_2022}. 
In addition to the pre-training aspect, finetuning is also explored in the literature. 
Specifically, there have been works that perform an analysis of which layers to freeze in the finetuning step \cite{digging_hoelzemann_2020}. 
Also, the choice of finetuning data can be made using mean distance measurements \cite{adapting_gong_2022}.  

In both the pre-training as well as finetuning stages, there are a number of training strategies that are incorporated to specifically address the domain shift. 
Joint training \cite{metier_chen_2020} is one such strategy, where losses associated with multiple tasks, like activity and user recognition, are combined and then optimized. 
The overall loss functions involved in such frameworks contain special losses like large-margin loss \cite{semanticdiscriminative_lu_2022}, MMD loss \cite{tasked_suh_2022}, sqaured MMD loss \cite{domain_hussein_2022}, domain confusion loss \cite{dmstl_zhu_2023}, domain classification loss \cite{dmstl_zhu_2023}, domain alignment loss \cite{domain_alajaji_2023}, triplet loss \cite{domain_alajaji_2023}, and supervised contrastive loss \cite{domain_wilson_2022}. 
Further, techniques like negative backpropagation with gradient reversal layer \cite{backdropout_ren_2018} and domain adaptive batch normalization \cite{incremental_mazankiewicz_2020} are also used to achieve the same goal. 

Parameter sharing can also be observed in more traditional solutions that follow self-training \cite{crossdomain_thukral_2023}, co-training \cite{improving_longstaff_2010}, ensemble learning \cite{personalized_reiss_2013}, active learning \cite{improving_longstaff_2010}, and pseudo labeling \cite{personalized_fu_2021}. 
Under the active learning paradigm, iterative \cite{study_oh_2021} and collaborative \cite{newnectar_civitarese_2019} versions have been explored, with decisions based on measures like least confidence, minimum margin, and maximum entropy. 
In ensemble methods, one-vs-all strategy \cite{smoke_nguyen_2015}, classifier weight updates \cite{personalized_reiss_2013}, and model calibration approaches \cite{toward_hong_2016} have been used. 
In addition to these commonplace approaches, a number of specific contributions using traditional methods have also been made. 
For example, decision trees \cite{crosspeople_zhao_2011}, feature incremental random forests \cite{novel_hu_2019}, ELM (along with its online version) \cite{crossperson_deng_2014} are also some of the traditional models that have been used in the transfer scenario.

We also note the parameter transfer works that are tailor-made to satisfy certain constraints that are imposed by the underlying methodology or the target application. 
In terms of the methodologies, soft parameter sharing \cite{domain_hussein_2022} (assuming a non-linear relationship between source-to-target transferred parameters) and cascaded learning \cite{transfer_du_2019} (iterative addition of trainable layers in model architecture) are the prominent examples. 
On the other hand, in terms of the target applications, federated learning \cite{federated_gudur_2020} and privacy preservation \cite{semisupervised_hashemian_2021} are the commonly targeted goals. 

\thomas{This entire section needs to be rewritten, I'm afraid. See my comments above (I don't want to repeat myself here.}

\subsection{Smart Homes}

\begin{figure}[]
  \centering
  \includegraphics[width=\linewidth]{Figures/smarthome_map.png}
  \caption{Map of the works in the smart home application domain. Here, the x-axis represents the year of publication and the y-axis represents the number of citations. Each connection represents a reference between the two works. A significantly lesser extent of exploration can be observed in the smart home application domain as compared to the ADL domain. \thomas{So, we want readers to compare the two diagrams. Why don't we put them next to each other then? The presentation style right now is very wasteful (w.r.t. space). Also: The captions are repetitive and the figures are nowhere referenced in the text. Again, this is paper writing 101 ...}}
  %\Description{}
  \label{fig:map_smarthome}
\end{figure}

Detecting activities in a robust and reliable manner has become a large area of interest \cite{hiremath2023lifespan}. 
With an increase in the number of IoT devices deployed in smart environments \cite{skocir2016activity}, the current trend in this domain is to incorporate multiple modalities of sensors like proximity (motion), wearable, physical (temperature and pressure), and contextual (RFID) sensors to develop frameworks for healthcare support \cite{amiribesheli2015review}, home assistance \cite{avgerinakis2013recognition}, energy management \cite{cottone2015user}, and security applications \cite{dahmen2017activity}.
Despite these promising opportunities, the underlying task of robust and reliable activity recognition is still yet to be fully solved, especially in real-world settings \cite{hiremath2023lifespan}.  

Firstly, most of the existing state-of-the-art works use sliding windows in their pipeline to avoid segmentation of sensor streams. \thomas{Nobody will agree to this (other than me). It is folk wisdom that sliding window is segmentation.}
This results in an overestimation of the performance \cite{tello2023too}. \thomas{What? No.}

Secondly, despite the availability of multi-modal data, many existing frameworks leverage only a single (or a small subset of) data modality in their frameworks, leaving the remaining data unused. \thomas{What? Where did you get that from? Wrong.}

Thirdly, the annotations performed on the prominent smart home datasets, for example, CASAS \cite{cook2012casas}, have classes like Cook, Relax, and Work that can have data points associated with a variety of actions performed by the subjects. \thomas{Are you talking about label ambiguity here or what?}
For instance, the activity of working may consist of simple actions like sitting on a desk for work, as well as more complex actions like vacuuming the floor.  
This interpretation of class labels may also vary from one smart home to another. \thomas{I don't follow this paragraph at all. What are you trying to say?}

Lastly, owing to the large variety in the layout of smart homes, sensor modalities, sensor locations, target activities, and subjects, learning transferable activity recognition models is inherently challenging. \thomas{Why?}

Therefore, a combination of all these challenges must be tackled while developing HAR as well as transfer learning frameworks in smart home settings. 
This trend is reflected in the relevant literature for smart homes, where the overall transfer learning framework consists of a combination of techniques for feature space alignment, label mapping, knowledge base, parameter, or instance transfer methods, and so on. 

\subsubsection{Feature-transfer}
Since multimodality is a de-facto challenge to address in smart homes, feature space mapping/alignment techniques are present in every transfer learning work in smart homes. 

The simplest method for this mapping is to perform sensor ID allocation \cite{cook2010learning}, profiling \cite{chiang2012knowledge}, or alignment using statistical measures like divergence (JSD) \cite{chen2017activity}, similarity measures (NGD) \cite{sukhija2018label}, sequence similarity measures \cite{guo2023transferred}, relative entropy \cite{hu2011transfer}, and correlation \cite{samarah2018transferring}.  
The use of these statistical measures in combination with domain knowledge driven \cite{sanabria2020unsupervised, ye2020xlearn}, Procrustes analysis based \thomas{?} \cite{feuz2017collegial}, and EM-based iterative approaches \cite{rashidi2011activity, rashidi2010activity, van2008recognizing, rashidi2011scaling} are also frequent in literature for intermediate feature space construction. 

Another prominent set of statistical approaches is to construct meta-features \cite{feuz2015transfer, van2010transferring} using compatibility functions \cite{wang2018activity, wang2019sensor}, Bayesian point machines \cite{diethe2015bayesian}, etc.\ to achieve a common source-target feature space. 
Along with the construction of such a feature space, the matching between the set of features is optimized via graph-matching methods \cite{lu2014instantiation}, genetic algorithm \cite{dillon2014heterogeneous}, and random forests \cite{sukhija2019supervised}.

Contrary to constructing a mapping between source/target features, the literature also consists of techniques like sparse coding \cite{dridi2022transfer} and ontological approaches \cite{chen2013ontology} that aim at constructing a dictionary of domain-invariant feature sets using data-driven \cite{hiremath2022bootstrapping} and knowledge-driven methods \cite{ye2014usmart}.  

More recently, the concepts from natural language processing and deep learning have also been successfully applied in learning feature space mapping. 
In particular, the incorporation of neural word embeddings \cite{azkune2020cross} and word2vec \cite{niu2020multi} has been explored in literature for common sensor data representations.  

The usage of neural networks like autoencoders (AE) \cite{rahman2022enabling}, graph AEs \cite{medrano2019enabling}, and bidirectional shift GANs \cite{sanabria2021unsupervised} has also been explored to obtain such data representations.
\thomas{You can't just dump everything into one giant paragraph. Who should read that?}


\subsubsection{Instance-transfer}
After feature transfer, the next most explored set of approaches for transfer learning in smart homes is instance transfer. 
The preliminary \thomas{Why "preliminary"? Don't insult the authors ...} works in this category perform sample weighing \cite{guo2023transferred, hu2011cross} and boosting \cite{inoue2016supervised} using similarity-based metrics. 
Another straightforward approach to implicitly perform instance transfer is via multi-view learning \cite{dillon2014heterogeneous} and its variant in co-training \& co-EM \cite{feuz2017collegial}, where intermediate data points, assumed by partitioning the feature sets, are used in a multi-view setup.  

In addition to these methods, we observe \thomas{Nope.} the following three major categories of instance transfer in the literature: (\textit{i}) synthetic data generation, (\textit{ii}) label space transfer, and (\textit{iii}) source domain selection. 
The idea behind synthetic data generation is to artificially create data points from the target domain, which has been attempted using survey-based rule/context-guided simulations \cite{ali2023user, azkune2015combining, ali2019improving} as well as GANs \cite{soleimani2021cross}. 

Next, in the label space transfer, the goal is to learn a mapping function between source and target label spaces, such that the instances from the source can be leveraged in the target domain training.
This is achieved using clustering (fuzzy \cite{polo2020domain} \& semantic clustering with label expansion \cite{ye2020xlearn}), NGD similarity \cite{hu2011cross}, pseudo-label \cite{sanabria2020unsupervised}, and discontinuous misplaced sequential mapping (DMSM) \cite{rashidi2009transferring} based methods. 

Finally, the source domain selection methods are used to prevent the degradation of transfer learning performance by choosing the optimal/closest source domains, which are selected using factors like classifier-induced divergence \cite{rashidi2011domain}, feature space similarity \cite{yu2023optimal}, semantic feature similarity \cite{niu2022source}, and domain parameters/metadata \cite{sonia2020transfer}.
\thomas{Again, this is poorly (if at all) linked to the intended application domain.}

\subsubsection{Parameter-transfer}
Lastly, in combination with feature and instance transfer, a few works based on parameter transfer have also been performed in smart home scenarios. 
Before diving into these works, we clarify that many of the feature and instance transfer works can also be considered under parameter transfer since, in many cases, the parameters learned in the process of feature extraction or instance transfer are in turn used for classification as well. 
For example, the ontological \cite{chen2013ontology, hiremath2022bootstrapping,ye2014usmart}, multi-view \cite{dillon2014heterogeneous, feuz2017collegial}, GAN \cite{sanabria2021unsupervised}  and AE-based \cite{rahman2022enabling,medrano2019enabling} approaches follow this pattern, where the parameters learned in the instance/feature transfer process are reused for classification as well. 
The standard setup of parameter transfer is to first train the classification model on one \cite{yu2023fine} or more \cite{niu2020multi} source domains, which is termed pre-training, followed by transfer to the target domain using either fine-tuning \cite{yu2023fine} or other processes like LDA-based inference \cite{kumar2018combining}. \thomas{Ok, now have introduced it a third time ... An appropriate way to link to the application domain would be to actually list and describe the particular source and target domains that are being use. But, no, we only vaguely list (again!) that there are source domains (whatever that would be) and we transfer to target domains (again, whatever that would be). How is that informative / useful?}
In this setup, classifiers like HMMs \cite{van2010transferring}, LSTMs \cite{yu2023fine}, dynamic Bayesian networks \cite{lu2013hybrid}, and hierarchical activity models \cite{rashidi2009keeping} are used in ensemble learning \cite{dillon2014heterogeneous} and shared-classifier \cite{ye2018slearn} scenarios. 

Finally, we also note a cognitive science based approach \cite{anjomshoaa2021transfer} to transfer learning that uses knowledge-graphs constructed using domain knowledge, as a mode of classification. \thomas{Care to explain?}

In terms of the types of sensors used, a majority of the works are based on the data collected by ambient sensors that are installed in smart home settings, consisting of predominantly binary motion sensors, temperature, and pressure sensors. \thomas{Should that not be clarified right at the beginning when we start talking about smart homes?}
Among them, a few works \cite{polo2020domain} only use binary motion sensors in their methodology, which makes the underlying transfer learning problem unimodal, which otherwise is inherently a multimodal task.

In addition to ambient sensors, a few other works \cite{alam2017unseen} assume the availability of wearable sensor data originating from smart home residents, which further complicates the challenge of varied sensing frequencies present among the sensors.

Finally, there have been some works that target specific use cases and use other data modalities like videos \cite{kumar2018combining} and web data \cite{hu2011cross}.
The review by Cust et al. \cite{cust2019machine} provides a comprehensive list of over 30 research articles that use distinct datasets collected by inertial sensors to recognize sports movements. 
However, they also point out a few drawbacks.
Many of those sensor datasets are collected using custom-built IMU units, which makes it harder to apply transfer learning. 
Moreover, the number of such sensors deployed in those settings ranges from 1 to 9, which can prove to be intrusive to the athletes.  
Finally, the amount and the coverage of the data collected are limited to the task at hand. 
For instance, the sensor attached to the tennis racquet cannot capture the entire range of an athlete's motion, and the data collected by it \textit{may} not generate transferable representations for other related sports. 
Because of these reasons, most of the prominent works in sports action recognition have leveraged the visual modalities (RGB, depth, and skeletal) \cite{host2022overview}. 

\thomas{My concerns mentioned above hold here as well.}


\subsection{Sports}

\begin{figure}[]
  \centering
  \includegraphics[width=\linewidth]{Figures/sports_map.png}
  \caption{Map of the works in the sports application domain. Here, the x-axis represents the year of publication and the y-axis represents the number of citations. Each connection represents a reference between the two works. The existence of small islands in this graph i.e. the graph is not very well connected, which is because of the different sports under consideration.\thomas{Another random figure with no link to the text at all?}}
  %\Description{}
  \label{fig:map_sports}
\end{figure}

With an increased interest in the competitive aspect of it, sports analytics has become an emerging research direction \cite{seshadri2019wearable, benlikaya2017can, wang2019ai}. 
Both body/object-worn inertial sensors \cite{nithya2021role} and visual (RGB) sensors \cite{wu2022survey} are used to recognize sports actions. 


\begin{comment}

Data-driven approaches are being developed to automate performance \cite{seshadri2019wearable} \& health \cite{benlikaya2017can} monitoring, strategy development \cite{wang2019ai}, movement classification \cite{borges2017validation}, and injury prevention \cite{kiernan2018accelerometer}.
In addition, applications like automated game assistance \cite{pan2020hierarchical}, highlight generation \cite{shroff2010video}, and sports commentary \cite{kanerva2019template} are also being targeted by researchers to further advance the field.
In all these applications, accurate recognition of human actions and activities lies at the core. 
\end{comment}


\begin{comment}
The workflow of recognizing sports actions and activities is very similar to the standard HAR setup, however, the challenges involved in it are different. 
First, we look at the data collection process from the perspectives of sensor installation, modalities, ease of collection, and required amounts.
In literature, both body/object-worn inertial sensors \cite{nithya2021role} and visual (RGB) sensors \cite{wu2022survey} are used to recognize sports actions. 
The review by Cust et al. \cite{cust2019machine} provides a comprehensive list of over 30 research articles that use distinct datasets collected by inertial sensors to recognize sports movements. 
However, they also point out a few drawbacks.
Many of those sensor datasets are collected using custom-built IMU units, which makes it harder to apply transfer learning. 
Moreover, the number of such sensors deployed in those settings ranges from 1 to 9, which can prove to be intrusive to the athletes.  
Finally, the amount and the coverage of the data collected are limited to the task at hand. 
For instance, the sensor attached to the tennis racquet cannot capture the entire range of an athlete's motion, and the data collected by it \textit{may} not generate transferable representations for other related sports. 
Because of these reasons, most of the prominent works in sports action recognition have leveraged the visual modalities (RGB, depth, and skeletal) \cite{host2022overview}. 
Visual sensors are less intrusive to athletes, cover more areas of sensing, and have the potential to produce better transferable representations.  
The survey by Wu et al. \cite{wu2022survey} lists more than 40 visual datasets in 10+ distinct sports, which demonstrates the wide acceptance of visual modality to perform sports action recognition and analytics. 
Yet, the usage of visual sensors comes at the cost of a unique set of challenges \cite{wu2022survey} like the occurrences of dense actions, fast movements, camera motion, occlusions, view-variance, etc.   
Also, the annotation of more complex and fine-grained sports activities requires domain expertise. 
Thus, the recent trend in sports action recognition is to address these challenges, prominently for the visual modality.  

After data collection, the next step in the workflow is to extract features and perform classification. 
Prior works using the data collected by inertial sensors extract features like acceleration magnitude \cite{adelsberger2013experts}, correlation \cite{anand2017wearable}, statistical features \cite{groh2015imu} (mean, variance, skewness, kurtosis), kinematic parameters \cite{jensen2015imu} (phase length, angle, velocity), domain frequency amplitudes \cite{kautz2017acquisition}, spatial features \cite{brock2017learning} (CNNs) and feed them to classifiers like LR \cite{anand2017wearable}, SVM \cite{adelsberger2013experts}, NB \cite{buckley2017binary}, RF \cite{groh2017classification}, DTW \cite{brock2017assessing}, MLP \cite{rassem2017cross}, CNN \cite{jiao2018multi}, LSTM \cite{anand2017wearable}, etc.
Whereas, in a majority of works in the visual modality, the tasks of feature extraction and classification are performed using the same architectural backbone. 
Although traditional models have been proposed that use features extracted using HOGs \cite{dalal2005histograms}, HOFs \cite{pervs2010histograms}, Bag of Words \cite{de2011evaluation}, and SIFT \cite{chen2009mosift}, their performances are not comparable to the ones obtained by applying deep learning approaches. 
To perform feature extraction and classification simultaneously, using deep learning, both 2D \cite{karpathy2014large} and 3D \cite{tran2015learning} convolutional models are extensively explored in the literature with backbone architectures like AlexNet \cite{donahue2015long}, VGG-16 \cite{srivastava2015unsupervised}, ResNet50 \cite{wang2018temporal}, InceptionNet \cite{carreira2017quo}, and ViT \cite{arnab2021vivit}.  
However, except for a very few \cite{karpathy2014large}, all the remaining works use a pre-trained backbone, typically on large vision datasets like ImageNet \cite{deng2009imagenet}, HowTo100M \cite{miech2019howto100m}, IG-65M \cite{ghadiyaram2019large}, etc. 
This is because, the features, especially the ones learned by the lower convolutional layers, are more likely to be transferable across domains and datasets for visual modality.  
Therefore, transfer learning via parameter sharing is widely used in sports action recognition tasks. 
\end{comment}

To understand the broader picture of Transfer Learning in sports activity/action recognition, we classify the works based on: (\textit{i}) sports, (\textit{ii}) sensor modalities, and (\textit{iii}) approaches. 
%We find that a majority of prominent studies \cite{tran2018closer, tran2015learning, donahue2015long, lin2019tsm, simonyan2014two} in this domain are carried out on generic datasets like UCF101 \cite{soomro2012ucf101}, Kinetics400 \cite{kay2017kinetics}, and its subsets, where not all action classes are exclusively related to sports.
We find that a majority of prominent studies \cite{tran2018closer, tran2015learning, donahue2015long} in this domain are carried out on generic datasets like UCF101 \cite{soomro2012ucf101}, Kinetics400 \cite{kay2017kinetics}, and its subsets, where not all action classes are exclusively related to sports.
%The remaining works are more targeted in nature, where transfer learning methods have been applied for specific sports like football \cite{luan2022action,cuperman2022end, jiang2016automatic, sen2022categorization, hong2018end, sen2022fine, stoeve2021laboratory, bose2023soccerkdnet}, tennis \cite{ullah2021attention, davar2011domain, sen2022sequence, farajidavar2011transductive}, volleyball \cite{gavrilyuk2020actor, shu2017cern, ibrahim2016hierarchical, ibrahim2018hierarchical, yuan2021spatio, qi2019stagnet}, hockey \cite{saveliev2019aggressive, santos2021efficient, mukherjee2017fight, rangasamy2020hockey, cai2019temporal, mumtaz2018violence, kecceli2017violent}, ice hockey \cite{tora2017classification, neher2018hockey, vats2019two}, badminton \cite{peralta2022badminton, binti2019recognition, rahmad2020vision}, e-sports \cite{apon2021action}, cricket \cite{sen2021cricshotclassify, khan2018deep, dixit2016deep, das2023deep, rahman2021deepgrip, kumar2019outcome}, skating \cite{liu2020fsd}, Olympic games \cite{mohamad2021olympic, liu2015simple}, traditional Bangladeshi sports \cite{sarma2021traditional}, frisbee \cite{link2022wearable}, gymnastics \cite{zan2023human}, etc.
The remaining works are more targeted in nature, where transfer learning methods have been applied for specific sports like football \cite{luan2022action,cuperman2022end}, tennis \cite{ullah2021attention, davar2011domain}, volleyball \cite{gavrilyuk2020actor, shu2017cern}, hockey \cite{saveliev2019aggressive, santos2021efficient}, ice hockey \cite{tora2017classification, neher2018hockey}, badminton \cite{peralta2022badminton, binti2019recognition}, e-sports \cite{apon2021action}, cricket \cite{sen2021cricshotclassify, khan2018deep}, skating \cite{liu2020fsd}, Olympic games \cite{mohamad2021olympic, liu2015simple}, traditional Bangladeshi sports \cite{sarma2021traditional}, frisbee \cite{link2022wearable}, gymnastics \cite{zan2023human}, etc.
%In terms of data modalities, most of the transfer learning contributions \cite{bo2020few, sargano2017human, patrick2021keeping, yang2022recurring, wang2018temporal, zhang2022tfcnet, neimark2021video} use video datasets, whereas, some works explore still images \cite{safaei2019still}, IMU sensors \cite{cuperman2022end, peralta2022badminton, qin2019cross, ding2018empirical, stoeve2021laboratory, xu2023integration, abdu2019versatl, link2022wearable}, and depth images \cite{zan2023human}.  
In terms of data modalities, most of the transfer learning contributions \cite{bo2020few, sargano2017human} use video datasets, whereas, some works explore still images \cite{safaei2019still}, IMU sensors \cite{cuperman2022end}, and depth images \cite{zan2023human}.
Finally, in terms of the transfer learning approaches, we witness a few glaring trends. 
Since a majority of the works are performed on visual data, the simplest transfer learning approach is to use a pre-trained backbone as the base feature extractor. 
The output features are then sent to a smaller custom network to extract domain-relevant features. 
Finally, this smaller network is fine-tuned on the datasets specific to the problem statement. 
Under this \textit{pretrain-big-finetune-small} approach, different kinds of pre-training have been explored in the literature. 
%The most common one is to use the ImageNet pre-trained classification model \cite{alamuru2022quick, bilal2022transfer, long2018attention, yue2015beyond, russo2019classification}. 
The most common one is to use the ImageNet pre-trained classification model \cite{alamuru2022quick, bilal2022transfer}. 
%Likewise, many works pre-train their backbones on large action recognition datasets like Sports-1M \cite{mishra2018generative,tran2019video, saveliev2019aggressive}, Kinetics-400 \cite{xie2018rethinking, jiang2019stm, li2021vidtr}, JFT-300M \cite{liu2022video}, and IG-65M \cite{wang2020makes}.  
Likewise, many works pre-train their backbones on large action recognition datasets like Sports-1M \cite{mishra2018generative,tran2019video}, Kinetics-400 \cite{xie2018rethinking, jiang2019stm}, JFT-300M \cite{liu2022video}, and IG-65M \cite{wang2020makes}.
%In addition to a variety of pre-training datasets, we also observe several pre-training tasks like pose estimation \cite{gavrilyuk2020actor, neher2018hockey, duan2022revisiting, duan2023skeletr, vats2019two}, activity recognition \cite{cuperman2022end}, object recognition \cite{herzig2022object, tora2017classification}, and optical flow estimation \cite{cai2019temporal}, which are performed in a supervised manner on large annotated datasets.
In addition to a variety of pre-training datasets, we also observe several pre-training tasks like pose estimation \cite{gavrilyuk2020actor, neher2018hockey}, activity recognition \cite{cuperman2022end}, object recognition \cite{herzig2022object, tora2017classification}, and optical flow estimation \cite{cai2019temporal}, which are performed in a supervised manner on large annotated datasets.
More recently, the pre-training task has also been performed in a self-supervised manner using contrastive learning \cite{tan2021vimpac} and different pretext tasks like masked image \cite{wang2022bevt}, video \cite{tong2022videomae}, feature \cite{wei2022masked}, and token \cite{tan2021vimpac} prediction. 

Apart from the works following the pretrain-then-finetune theme, there have been a number of instance, feature, and parameter transfer contributions. 
In instance transfer, multi-subject augmentations \cite{peralta2022badminton}, source domain selection \cite{qin2019cross}, and skip-gram based label transfer \cite{gan2015exploring} are performed. 
Under feature transfer, conventional methods (e.g.\ feature re-weighing, translation, and scaling \cite{farajidavar2011transductive}, per-feature linear transform \cite{davar2011domain}, and sparse coding \cite{zhu2011sparse}) as well as deep learning based methods (e.g.\ dual many-to-one encoder \cite{xu2016dual}, MMD \& Wasserstein distance \cite{ding2018empirical}, and data augmentation \cite{xu2015semantic} based) are explored. 
Lastly, in parameter transfer works, architectural contributions like Graph neural networks \cite{duan2023skeletr}, energy based deep belief networks \cite{roder2021actions}, temporal segmentation networks \cite{liu2015simple}, 3-stream CNN-LSTM networks \cite{zan2023human}, and lead exceed multimodal network \cite{gan2016you} are present.
Standard domain adaptation methods like MMD loss and gradient reversal layer based domain adaptive neural networks and deep domain confusion networks are also explored \cite{xu2023integration}.
A special type of loss function for scene invariance is also proposed for better generalization across background scenes \cite{choi2019can}.
Along with pre-training, some works perform subject-specific finetuning for personalization \cite{peralta2022badminton}.     

\thomas{This subsection is totally random and I have no idea why this is in here.}
\begin{comment}
Barring these works that follow the \textit{pretrain-big-finetune-small} trend, other studies employ transfer learning methods custom-made for the challenges involved.
Peralta et al. \cite{peralta2022badminton} construct a generalized action recognition model using multi-subject augmented data, followed by subject-specific finetuning for personalization.
Qin et al. \cite{qin2019cross} perform source domain selection and construct spatial \& temporal adaptive features.
Davar et al. \cite{davar2011domain} estimate a transformation that matches the source and the target class-wise probability distributions to perform domain adaptation. 
Xu et al. \cite{xu2016dual} develop dual many-to-one encoders to align feature vectors in a common vector space.
Ding et al. \cite{ding2018empirical} conduct an empirical study to compare the transfer learning performance using CNNs, maximum mean discrepancy, domain-adversarial neural network, and Wasserstein distance based methods. 
Gan et al. \cite{gan2015exploring} leverage the semantic inter-class relationships between known and unknown actions using a skip-gram model, followed by performing label transfer.
Roder et al. \cite{roder2021actions} propose to use energy-based spectral deep belief network to map action-to-event knowledge. 
Liu et al. \cite{liu2015simple} use a keyframe sampling based temporal segment network, which can be used to perform transfer from single to dual-subject skating scenarios. 
Zan et al. \cite{zan2023human} use a 3-stream CNN-LSTM model to perform cross-subject evaluations. 
Xu et al. \cite{xu2023integration} propose a fast and robust transfer approach based on domain adaptive neural networks, deep domain confusion networks, and an adaptive classifier based on online sequential extreme learning machine. 
Wang et al. \cite{wang2017internal} design an internal transfer learning strategy using a sub-data classification method. 
Xu et al. \cite{xu2015semantic} propose a self-training and data-augmentation based mapping between visual features and semantic attributes. 
Duan et al. \cite{duan2023skeletr} design a graph convolutional network based SkeleTR framework, which can be pre-trained on multiple tasks prior to performing action recognition. 
Zhu et al. \cite{zhu2011sparse} encode spatio-temporal gradient features using a trained dictionary of features obtained via sparse coding. 
Farajidavar et al. \cite{farajidavar2011transductive} employ feature re-weighing, translation, and scaling techniques on HOG3D features to adapt domain shifts in tennis games.
Choi et al. \cite{choi2019can} include scene type adversarial loss and scene masking in their training pipeline to reduce the effect of background scenes on activity inference under domain shift. 
Gan et al. \cite{gan2016you} design a Lead Exceed neural network to incorporate relevant web images and videos in the pre-training phase for better generalization. 
\end{comment}

\begin{comment}

\subsection{Surveillance}
~\cite{khurana2018deep} <- Survey \\
\textbf{special mentions apart from general outline:}
\begin{enumerate}
    \item Images and videos are most commonly used, however, thermal and depth cameras are also used. 
    \item Indoor vs Outdoor environments. 
    \item Background elimination task required (non-HAR task)
    \item recognition of subjects or types of subjects. 
    \item robustness to orientation, overlap, lighting conditions required. 
    \item segmentation and tracking applicable 
\end{enumerate}

\subsection{Healthcare}
~\cite{zhang2020personalized} <- Thesis \\
\textbf{special mentions apart from general outline:}
\begin{enumerate}
    \item Settings similar to ADL or Smart homes, but focus on fitness and health monitoring. 
    \item Outlier activities: less data, cannot be simulated
    \item incorporation of domain knowledge and heuristics required 
    \item performance cannot be compromised in certain cases: trade-off between false positives and false negatives. 
    \item Explainability required. 
    \item on top of recognition, assistance and providing directions/suggestions is important. 
\end{enumerate}
\end{comment}


==> approaches.tex <==
%In the previous section, we looked at the categorization of Transfer Learning from the problem perspective, where the distinctions are made based on problem characteristics like availability of source/target labels, similarity in source/target tasks, etc. 
In this section, we focus on the solution perspective and provide details on different methodologies employed under (\textit{i}) Instance-transfer, (\textit{ii}) feature-transfer, (\textit{iii}) parameter-transfer, and (\textit{iv}) knowledge-transfer, as shown in Figure~\ref{fig:TL_approaches}. 
%make distinctions based on the type of methodology employed. 
%As we saw in the previous section, any machine learning problem can be well-defined by specifying a tuple of a domain ($D$) and a task ($T$). \thomas{Not "we". Also: Why parentheses?}
%In a transfer learning settings, we have a pair of source ($D^s, T^s$) and target ($D^t, T^t$) problems and the goal is to reuse/transfer the \textit{knowledge} gained from solving the source problem in the target problem. 
%From the solutions perspective mentioned earlier, the types of Transfer Learning depend on the kind of \textit{knowledge} that is transferred across domains. \thomas{Still not sure that dual view (problem/solution) is necessary / adds much.}
%The possible candidates for this transfer of knowledge are in the form of data instances, features, learned parameters, and domain knowledge. 
%This gives rise to four categories of Transfer Learning: (\textit{i}) Instance-transfer, (\textit{ii}) feature-transfer, (\textit{iii}) parameter-transfer, and (\textit{iv}) knowledge-transfer, as shown in Figure~\ref{fig:TL_approaches}. 
Specifically, we provide a formal background on the most prominent
%\thomas{Why only some? Begs the question on how we selected. Why not "the most prominent"?} 
methodologies explored in each of the categories. 
To understand their mathematical background, we encourage the readers to refer to the Appendix section in supplementary materials. 
%It should be \thomas{Well then do it (the noting) ...} noted that we provide the mathematical background for them in our supplementary material. 
%This section only contains the descriptions of these methods. \thomas{"Only" sounds very negative. Last sentence needed?}


 

\subsection{Instance Transfer}
\label{subsec:Instance_Transfer}

Instance transfer 
%broadly \thomas{Why "broadly"? Be specific and go easy on those adjectives. They typically don't add much other than fluff.} 
refers to a methodology that reuses the data instances from the source domain $X^s$ in solving the target domain task $T^t$. 
The most common interpretation of this approach is to re-weight the data points based on a similarity/importance metric and transfer them in the learning process of the target domain. 
Approaches like boosting~\cite{rokni2018autonomous}, sample weighing~\cite{shen2023transfer} using distribution matching~\cite{ding2018empirical} followed by similarity-based instance addition/removal~\cite{framework_wen_2017} are the commonly used ones to perform such instance transfer. 
%We call \thomas{"call"?} such approaches explicit instance-transfer methods since they follow the weighted data point interpretation. 
In addition to that, there also exist approaches that implicitly make use of the source data points for performing synthetic data generation \cite{ali2023user, soleimani2021cross}, label space transfer \cite{polo2020domain, ye2020xlearn}, and source domain selection \cite{rashidi2011domain, yu2023optimal}. 
Such approaches do not weight individual data points, rather follow a different suit entirely.  

%In addition to that, we also observe \thomas{Where? In the observatory? Language ...} some \thomas{"some"?} implicit methods like synthetic data generation \cite{ali2023user, soleimani2021cross}, label space transfer \cite{polo2020domain, ye2020xlearn}, and source domain selection \cite{rashidi2011domain, yu2023optimal} that perform instance transfer without explicit re-weighing of individual data points.
%Below, we describe in detail each of these methods. 

\subsubsection{Instance Weighing}
The general idea behind instance weighing is to assign importance to source data instances $x_i$, in the form of weights $w_i$, to denote their usefulness in the transfer process. 
Broadly, there are two ways in which this weight assignment is performed: (\textit{i}) based on similarity of data instances \cite{zhang2018importance,guo2023transferred} and (\textit{ii}) based on extent of misclassification \cite{shu2019transferable,chakma2021activity}. 
The similarity between source and target instances is often measured using methods like kernel mean matching \cite{gretton2009covariate}, density ratio estimation \cite{sugiyama2012density}, sensor similarity \cite{chiang2012knowledge}, feature similarity \cite{chiang2017feature}, sensor sequence similarity \cite{guo2023transferred}, mutual information \cite{novel_hu_2019}, maximum mean discrepancy (MMD) \cite{feature_chen_2021}, and log likelihood \cite{importanceweighted_hachiya_2012}.
The other way of assigning weights to data instances is by using a classifier's extent of misclassification as a proxy for the importance of that data instance. 
In particular, this extent of misclassification is measured using cross-entropy loss, domain classification loss, meta classification loss, and confidence \cite{swladapt_hu_2023}.
Figure \ref{fig:instance_transfer_approaches} provides an overview of these instance weighing methods. 


Boosting is one of the common ways in which data samples are weighted in this manner. 
Methods like AdaBoost \cite{freund1999short} maintain a distribution of weights over the data instances, which gets updated based on the performance (mis-classifications) of the weak learner.
This can be extended in a transfer learning setup in the form of TrAdaBoost and TransferBoost \cite{venkatesan2011study}. 
In TrAdaBoost, the mis-classified data instances on the target domain are given more weightage, whereas, the same for the source domain are given less weightage, which implicitly weights the source data points for their usage in target classifications. 
On the other hand, TransferBoost extends the boosting method to a multi-source framework, where individual source-to-target pairs get weight updates as per AdaBoost, which are further scaled and normalized as per the contribution of each source domain towards target classification. 

\begin{figure}[]
  \centering
  \includegraphics[width=\linewidth]{Figures/instance_transfer.pdf}
  \caption{Overview of the instance transfer approaches, where the majority of the solutions fall into the four mentioned categories i.e. instance weighing, source domain, selection, synthetic data generation, and label space transfer. Contributions belonging to each category are listed below the labels. 
  %\thomas{Again no referencing from text ...}
  }
  %\Description{}
  \label{fig:instance_transfer_approaches}
\end{figure}

\subsubsection{Source Domain Selection}
While instance weighting assigns importance scores (weights) to individual data instances, the source domain selection approach follows a similar suit to choose compatible domains to perform the transfer in a multi-source setting. 
Since this problem statement is similar to instance weighing, in essence, similar kinds of approaches are used here.
Different kinds of domain distances such as global domain \& sub-domain distance \cite{dmstl_zhu_2023}, semantic \& kinetic distance \cite{deep_wang_2018}, XHAR distance \cite{xhar_zhou_2020}, stratified domain distance \cite{crossposition_chen_2019} etc. are proposed in the literature that depend on similarity between data instances, features, or domain characteristics, as shown in Figure \ref{fig:instance_transfer_approaches}. 
The feature space distances are more concerned with factors like overlap of sensing modalities \& positions \cite{yu2023optimal} and semantic measures \cite{niu2022source}, whereas, domain parameters are more concerned with subject-specific, environment-specific, and routine-specific domain characteristics \cite{sonia2020transfer}.    

\subsubsection{Label Space Transfer}
Label space transfer is a type of methods, where a mapping function between the source and the target label sets is learned. 
This ensures that source instances can also be used in target domain training in a supervised manner, owing to the newly assigned target domain labels. 
The way in which this label space mapping function can be learned is via mapping the similar data instances, clusters, or communities from both domains followed by transferring the labels by optimizing some kind of a distance/similarity measure. 
This process is performed using these three approaches: 
%\thomas{All three in combination or or one these? Ambiguous.}
(\textit{i}) using similarity/distance measures, (\textit{ii}) by clustering-based mapping, (\textit{iii}) by constructing a graph mapping problem.
In the first category, measures like cosine similarity \cite{evaluating_wijekoon_2020}, RBF kernel based similarity \cite{personalized_bettini_2021}, normalized Google Distance (NGD) \cite{hu2011transfer}, Wasserstein distance \cite{deeptranshar_kumar_2023}, etc. are used. 
Such measures, like centroid distance \cite{collaborative_kong_2020}, can also be used alongside clustering, where data instances are initially clustered and then distances between source and target clusters are used in similarity calculations for label mapping. 
Following this approach, fuzzy \cite{polo2020domain} and semantic \cite{ye2020xlearn} clustering have also been explored for label space transfer. 
Finally, label space mapping can be viewed as graph matching problem \cite{plugnlearn_rokni_2016}, where the goal is to optimize a cost function (formed using similarity/distance measures) by performing mapping between instances/clusters/communities. 
Figure \ref{fig:instance_transfer_approaches} provides an overview of these label space transfer methods. 

\subsubsection{Synthetic Data Generation}
Unlike traditional instance transfer, where source instances are weighted and reused in target model training, the key idea here is to use data instances outside the target domain (or their properties) for constructing artificial data instances in the target domain. 
Literature consists of two types of such synthetic data generation methods: (\textit{i}) leveraging other data modalities (or their pre-trained models) and (\textit{ii}) generative methods. 
In the literature, models trained on other data modalities like videos \cite{kwon2020imutube}, skeletal maps \cite{novel_fan_2022}, and motion capture data \cite{learning_xia_2021} are used to generate synthetic IMU data. 
It should be noted that these approaches could also be considered under parameter transfer.
However, we include them under instance transfer because the main motivation of these approaches is to extract the motion characteristics that are hidden in the \textit{data instances} of the other modalities. 
There are also methods that generate synthetic data without any parameter sharing. 
Such methods often rely on user surveys (for personalizing the generated data), rule-based systems, and simulators \cite{ali2023user}.  
Moving on to the other type i.e. generative models, generative adversarial networks (GANs) \cite{soleimani2021cross} and their variants \cite{generic_soleimani_2022} have been explored in the literature to generate synthetic data for the target domain. 
The idea is to use a generator network that inputs source data points and a noise vector and produces fake data points, which the discriminator tries to classify. 
The loss function for the generator network consists of the discriminative loss as well as the source classification loss, which is usually applied during cross-domain transfers.  
Lastly, an indirect method to produce synthetic data is by using data augmentations \cite{semanticdiscriminative_lu_2022}. 
The goal here is to produce target domain data instances that follow the domain constraints.  
Figure \ref{fig:instance_transfer_approaches} shows these discussed methodologies for synthetic gata generation. 

%\thomas{MAde it up to here. The technical stuff is much better than the higher level narrative. We still need to think about the added value this survey will provide to readers. It looks like the paper could do with some more illustrations. We also need to make clear early on what will be found in the appendix (I know we had agreed to not have this in for my review right now, so this is just a reminder.}
\subsection{Feature Transfer}
\label{subsec:feature_transfer}
Feature transfer is a type of transfer learning method, where data instances from the source and the target domain are mapped onto a common feature space.
The intuition behind these methods is to enable the source classifier to perform inference on the target domain after the data instances are mapped accordingly. 
The common feature space can simply be the target space, in which case, the source data can be mapped to the target feature space (or vice versa) and a common model can be learned. 
Another way is to learn an intermediate feature space, different from both source and target domains, which can be \textit{designed} in a way that boosts the transfer learning performance. 
In the literature, two themes of such feature transfer approaches are found: (\textit{i}) conventional algorithmic approaches and (\textit{ii}) deep learning based approaches. 
%\thomas{Make that passive voice?}

\begin{figure}[]
  \centering
  \includegraphics[width=\linewidth]{Figures/feature_transfer.pdf}
  \caption{Overview of the conventional feature transfer approaches. 
  These approaches optimize various statistical measures associated with the distribution of data instances to construct the intermediate feature spaces. 
  }
  %\Description{}
  \label{fig:feature_transfer_approaches}
\end{figure}


\subsubsection{Conventional Algorithmic Approaches}
In this category, we include the conventional algorithms designed to perform feature extraction, which are leveraged in the feature transfer settings as well.
We first start with dimensionality reduction techniques like principal component analysis (PCA) \cite{achieving_lago_2020} and latent Dirichlet allocation (LDA) \cite{framework_wen_2017} based feature transfer. 
\thomas{In general: We need to write out those abbreviations the first time we introduce them. Here in particular it can be misguiding to not do so: LDA as in Latent Dirichlet Allocation or as in Linear Discriminant Analysis? The latter is much closer to PCA (it is basically PCA with class information) than the former ...}
PCA is an unsupervised algorithm that applies an orthogonal linear transformation to the data instances in order to project them on a lower dimensional feature space, where variance along the new dimensions (principal components) is maximized. 
On the other hand, LDA is a hierarchical model that is commonly used for topic modeling, where documents are modeled by assuming a multinomial distribution over latent topics, which are further modeled using a similar distribution over words. 

\thomas{Add paragraph breaks -- you have a strong tendency to dump a lot of text into giant paragraphs, which are then very hard to read.}
Now, \thomas{Stop using the word "now" as you would in a talk ...} in the case of sensor data, because of multi-dimensionality and continuous feature spaces, making such an assumption is not only infeasible but also prone to overfitting due to a large number of parameters to learn. 
Thus, methods like AdaBoost are used as proxies to calculate the predictive likelihood in LDA \cite{learning_wen_2017}.
While reducing dimensions, certain objectives are considered.  
For example, after the projection of source and target data instances on the reduced subspace, the distance between their distributions should be minimal. 
However, similar to PCA, the variance across new components should also be higher for smooth inference.

To achieve both goals simultaneously, transfer component analysis (TCA) 
%\thomas{?}
\cite{unsupervised_barbosa_2018} uses an MMD-based
%\thomas{?} \sourish{defined it earlier now}
measure for distribution alignment and a parametric kernel map-based objective for structure preservation, which are optimized together. 
In addition to using MMD for calculating domain alignment, measures like Bregman divergence \cite{si2009bregman} are also used. 
In particular, subspace alignment (SA) \cite{unsupervised_barbosa_2018} attempts to learn a transformation that projects the source instances onto a subspace that is closer to the target domain in terms of Bergman divergence. 
It does so by using the covariance matrix between the source and the target eigenvectors. 
Another way to look at domain alignment is by minimizing the distance between the covariance matrices of the source and target feature vectors. 
This is performed in correlation alignment (CORAL) \cite{transfer_li_2022}, where an analytical solution to the aforementioned problem is presented. 

All these methods work on the global properties of the domain i.e. by considering \textit{all} the data instances present in the domains. 
Next \thomas{"Now" again ...}, we look at locally linear embedding (LLE) 
%\thomas{?}
\cite{personalized_saeedi_2018}, which considers only the $k$-nearest neighbors around each data instance and tries to reconstruct each data point linearly using this neighborhood.  
Thus, LLE learns a weight matrix denoting reconstruction weights corresponding to each data instance pair. 
The corresponding optimization problem is solved using singular value decomposition (SVD)
%\thomas{?} 
and eigenvector-based techniques. 

Lastly \thomas{"now" ...}, we look at \thomas{not a talk ...} sparse coding \cite{unlabeled_bhattacharya_2014}, which looks at this problem from a dictionary-learning perspective. 
Unlike the previous methods, it tries to increase the dimensionality of this intermediate space by learning an over-complete set of vectors. 
This is done by formulating an optimization problem based on reducing the reconstruction error and increasing the sparsity in the learned vectors. 

\subsubsection{Deep Learning based feature transfer}
In the conventional feature transfer approaches, we can see \thomas{Not a talk ...} that the source and target data instances are mapped to an intermediate space by applying transformations. 
Deep neural networks can also be seen as cascaded sequences of non-linear transformations, where the output of each hidden layer is a projection of its previous layer onto a different subspace. 
Moreover, neural networks can be designed to handle even discrete feature spaces and project data points onto a continuous space, where it becomes easier to perform transfer and learn classifiers.
Hence, neural networks can be seen as a way of modeling the required non-linear transformations that are applied to perform feature transfer. 

The transformations applied by neural networks depend on two factors, namely the model architecture and the loss function of the network.
In terms of model architecture, autoencoders (AE) \cite{rahman2022enabling}, convolutional neural networks (CNN) \cite{sensehar_jeyakumar_2019}, long short term memory units (LSTM) \cite{activity_okita_2018}, bidirectional generative adversarial networks (Bi-GAN) \cite{contrasgan_sanabria_2021}, and attention weights \cite{mars_pei_2021} have been tested to perform the non-linear transformations. 
The parameters present in these architectures are trained using various loss functions like cross-entropy loss, reconstruction loss \cite{rahman2022enabling}, domain discrimination loss \cite{semisupervised_chakma_2022}, MMD loss \cite{chang2020systematic}, Jensen–Shannon divergence (JSD) loss \cite{augtoact_faridee_2019}, NGD loss \cite{sukhija2018label}, etc. 
%\thomas{Abbreviations again ...}

The cross-entropy and reconstruction losses are applied to take into account the performance of the classifier and the ability to preserve the characteristics of data in the embedding space, respectively. 
However, they act as necessary but not sufficient conditions in order to perform the transfer. 
These required additional conditions are imposed by the remaining special loss functions. 
For instance, the domain discrimination loss directs the training toward learning a classifier using the features projected on the intermediate space. 
Then, it is fed to a gradient reversal layer \cite{rahman2022enabling}, which dictates weight updates in the opposite gradient direction, which causes the architecture to \textit{not} learn the domain-specific characteristics. 

While this loss depends on the performance of the domain classifier, the MMD loss depends entirely on the distribution characteristics of both domains.
Specifically, it is a distance measurement between the means of the projected dimensions of source and target data on the intermediate feature space. 
Similar to using the means of these projected dimensions as a proxy for (dis)similarity of distributions, Kullback-Leibler (KL)
%\thomas{?} 
divergence can also be used instead. 
However, KL divergence is not symmetric in nature and has no upper bound, which is why, a symmetric and bounded version is used in the form of JSD. 
Finally, we also have \thomas{Not a talk ...} loss measures designed for the supervised transfer of feature spaces, like the NGD-based measure, which enforces the distributions of similar labeled instances to be aligned. 




\subsection{Parameter Transfer}
\label{subsec:parameter_transfer}

Parameter transfer refers to the type of transfer learning method, where the parameters \textit{learned} in the source domain training are reused in the target domain training. 
The assumption behind using these approaches is that there exists domain-specific and activity-specific information that is embedded in the learned parameters.
The goal here is to transfer the parameters that are domain agnostic or activity specific such that it can assist the target domain classification.

Traditional parameter transfer approaches rely on techniques like self-training \cite{improving_longstaff_2010}, co-training \cite{improving_longstaff_2010}, active learning \cite{improving_longstaff_2010}, pseudo labeling \cite{personalized_fu_2021}, and ensemble learning \cite{personalized_reiss_2013} based on classifiers like extreme learning machines (ELM)
%\thomas{?}
\cite{crossperson_deng_2014}, decision tree \cite{crosspeople_zhao_2011}, random forest \cite{novel_hu_2019}, hidden Markov models (HMM) \cite{van2010transferring}, Bayesian network \cite{lu2013hybrid}, etc.  

However, since the inception of deep learning, the domain of parameter transfer has been shifted to using neural networks, where it is easier to learn and transfer only specific parameters across domains. 
In such approaches, the commonly used pipeline is to perform pre-training on the source domain, to learn the required parameters, followed by finetuning on the target domain, where they are transferred and partially updated to make them suitable for the target domain. 
In the pre-training step, the source domain training can be performed in a supervised \cite{crossdomain_khan_2022}, semi-supervised \cite{chakma2022semi}, un-supervised \cite{autonomous_rokni_2016}, or self-supervised \cite{haresamudram2022assessing} way. 
The next step is to choose \textit{which} parameters to transfer to the target domain \cite{digging_hoelzemann_2020}.
After transferring the parameters, they are finetuned using the labeled data available in the target domain. 
The majority of contributions in the parameter transfer approaches lie in the pre-training step, whereas, only a handful of works target the parameter transfer \cite{transfer_an_2020} and fine-tuning steps \cite{adapting_gong_2022}. 
Through the subsequent paragraphs, we focus on the following three major themes observed in the works focusing on the pre-training aspect. 

\subsubsection{Neural Network Architecture}
To perform pre-training, different types of neural networks like AE (fully connected \cite{untran_khan_2018}, convolutional \cite{haresamudram2022assessing}, and variational \cite{latent_qian_2021}), CNN \cite{cnn_chikhaoui_2018} and its variant architectures like Bayesian CNN \cite{personalizing_akbari_2020}, ResNet \cite{crossdataset_gjoreski_2019}, and GoogleNet \cite{physical_ataseven_2022}, recurrent networks (including GRU \cite{recurrenthar_kumar_2022}, LSTM \cite{activity_okita_2018}), transformers \cite{strangan_faridee_2021}, and hybrid architectures (CNN-LSTM \cite{deep_wang_2018}, graph networks \cite{deep_yan_2022}, generative networks \cite{soleimani2021cross}), etc. have been explored. 

In AEs, the aim of the network is to learn parameters that can encode the input data into a lower-dimensional subspace (in the form of an encoder) and then reconstruct it (in the form of a decoder). 
The non-linear transformations that are applied to perform this encoding and decoding are in the form of fully-connected and convolutional layers. 
Variational AE, on the other hand, model the process of encoding and decoding as learning a distribution of the input data over the intermediate space. 
Thus, in addition to minimizing the reconstruction error, variational AEs also have a regularization term of the learned distribution in their loss function. 

In CNNs the idea of parameter sharing is used. 
Unlike fully-connected layers, where a weight between each pair of hidden neurons is separately learned, CNNs learn a set of weight kernels that are convolved over the lengths of data instances such that spatial features can be learned.
CNN architectures vary in terms of the depth of the network (number of convolutional layers/blocks), number of kernels, their dimensions, additional connections (e.g. skip connection), etc. 
Similar to variational AEs, CNNs can also incorporate variational inference in the form of Bayesian CNNs. 
Instead of learning weight values in the kernels, they can be replaced with parameters of a probability distribution, which helps in avoiding overfitting of the model.
As CNN architectures are intended to learn spatial features, recurrent architectures are targeted for learning temporal features. 

A simple RNN \thomas{?} architecture is a bi-directional neural network that processes the input from the current timestamp as well as the output from the previous hidden state, to learn temporal context.
Such architectures often encounter the problem of vanishing gradients, which is addressed in architectures like GRUs and LSTMs. 
The LSTM unit is a gated architecture, consisting of input, forget, and output gates that are capable of learning long-term dependencies. 
On the other hand, the GRU unit is  a modification of the LSTM unit, where the functionalities of the input and the forget gates are combined in an update gate, resulting in fewer parameters to learn. 
Although these architectures address the vanishing gradient problem, they still process the input sequentially, which inherently results in missing out on long-term context. 
Also, because of the sequential processing of the input, there exists a context window beyond which, it gets harder to process temporal dependencies. 

The solution to this problem is to process the entire input sequence at once, in parallel, which is performed in transformer networks. \thomas{Ref?}
Here a self-attention mechanism is employed, where each input token from the sequence gets attended to every other token such that long-term context can be learned. \thomas{Not sure a "lay" person would understand this?}

In addition to the aforementioned architectures, the literature consists of many hybrid models that contain a combination of fully connected, convolutional, and recurrent layers in the neural network design. 
Also, some architectures contain additional top-level structures that facilitate the learning of special kinds of features. 
One such type of neural network is graph neural networks, which consist of nodes (containing features) and connections (representing relation between them). 
These encoded features are trained using message passing algorithms, where information is gathered from the neighbors of a node, followed by updating the parameters, and finally, propagation of this information in the subsequent graph network. 

Lastly, we look at \thomas{Not a talk ...} GANs, which consist of a generator and a discriminator architecture trained in an adversarial manner. 
The generator uses a noise or a latent space vector to generate synthetic data instances, which are classified by the discriminator as real or fake. 
After training these models until equilibrium, without any mode collapse, the generator network can be used to perform target domain data generation as well as classification. 

\thomas{This is all nice but rather superficial (also not much referencing going on here) -- so, I wonder what the actual value is that we add here?}

\subsubsection{Training Strategies}
The training of neural networks is guided using two factors, namely the loss function and the optimization. 
Designing these two factors can direct the training process towards learning specific kind of features, which in our case are the features that can be transferred across domains. 

In the construction of the overall loss functions, different kinds of losses are often combined, each having a different purpose. 
Downstream classification performance is the most important factor, to determine which loss shall be included. 
In addition, there are other kinds of losses that depend on the predictions of the model. 
For instance, the large margin loss \cite{semanticdiscriminative_lu_2022} is typically used for generalization purposes, where the intention is to learn decision boundaries that can classify data instances with larger margins (high confidence). 

Another important aspect of classifier predictions is their inability to differentiate between the projections of the source and target domains. 
This is achieved using domain classification and domain confusion losses \cite{dmstl_zhu_2023}, which represent the classification error and cross-entropy between the distribution of class labels and predictions, respectively. 

In addition to this, often there are regularization terms applied to the parameters and their distributions. 
For example, MMD-based measures (MMD \cite{domain_qin_2022} and squared MMD \cite{domain_hussein_2022}) in the form of domain alignment losses are applied so that the source and the target domain feature distributions align closer to each other. 

Another philosophy in loss function design is to direct training such that \textit{similar} data instances have feature representations closer to each other. 
This is achieved using triplet \cite{endtoend_ye_2021} and contrastive loss \cite{contrasgan_sanabria_2021}. 

Finally, we also have \thomas{Not at talk ...} multi-source \cite{multisource_wilson_2020} and multi-task \cite{multitask_saeed_2019} training setups, where corresponding losses are jointly optimized. 
In a multi-source setup, the same task is performed on a number of source domains so that a wide range of data-specific features can be learned.  
In a multi-task setup, on the other hand, related tasks like activity and subject recognition \cite{metier_chen_2020} are simultaneously performed, using shared features.  

Along with loss function design, there have also been works that focus on the optimization aspect. 
For instance, the incorporation of gradient reversal layer \cite{multisource_wilson_2020} is commonplace, especially in the presence of some kind of domain discrimination related losses. 
This layer simply reverses the sign of gradient, which forces the network to \textit{not} learn domain-specific features. 

Another major contribution in this area is domain adaptive batch normalization \cite{mazankiewicz2020incremental}, which is based on the fact that the batch normalization layer encodes domain-specific information. 
The idea of batch normalization is to keep the input distribution to each layer constant by replacing the output activations of previous layers with their standardized values. 
Thus, to perform transfer, instead of using exponentially weighted average to compute statistics, the entire test domain data is used to impose the same distribution across source and target domains. 
Thus, the network can then produce representations in a subspace where both source and target distributions are similar. 

\subsubsection{Training Setups}
Aforementioned parameter transfer approaches are characterized by their training setups, which depend on the problem setting and the constraints involved. 
For example, supervised pre-training can be performed in the presence of large labeled source domains. 
Similarly, multi-source training can be performed when multiple source domains are present. 
However, the most prominent research direction is to perform this pre-training without using labels. 
In addition to the requirement of labeled datasets, there are drawbacks to using label information in pre-training. 
Using class labels in training results in learning domain-specific features, which are not transferable. 
Thus, unsupervised and self-supervised methods are commonly deployed to extract more generic features. 

Self-supervised learning is a paradigm, where the source of supervision for training comes from the unlabeled dataset itself. 
In particular, a pretext task is constructed, which is different from the main downstream task. 
In this pretext task, usually, a transformation is applied to the unlabeled data, and the aim is then to recognize the properties of the applied transformation. 
For instance, in the pretext task of masked reconstruction \cite{haresamudram2020masked}, a transformation of data masking is applied to the unlabeled data, and the aim is to predict the masked data values using the remaining portion as context. 
Likewise, pretext tasks of sensor modality classification \cite{deep_li_2020}, sensor context detection \cite{autonomous_rokni_2016}, data reconstruction \cite{haresamudram2022assessing}, multi-task transformation prediction \cite{multitask_saeed_2019}, and future timestamps prediction \cite{haresamudram2021contrastive} are explored in the  literature. 
Along with pretext task based self-supervision, contrastive learning can also be applied to learn representations. 
As stated earlier, contrastive learning aims at generating similar representations of similar data instances, using InfoNCE loss \cite{haresamudram2021contrastive}.
SimCLR, SimSiam, and BYOL are contrastive learning based setups explored in the literature \cite{haresamudram2022assessing}. 

These supervised and un-/self-supervised training setups are conventional in the sense that they assume the availability of pre-training and inference data all at once.  
However, that is not the case in many practical scenarios, where training and inference need to be performed on streaming sensor data. 
In such cases, the continual/ incremental learning setup comes into the picture. 
Specifically, the learning algorithms in this setup are targeted for sequential learning from a sensor stream or a dynamic environment. 
This is achieved using techniques like replay \cite{online_sztyler_2017}, dynamic classifier learning \cite{lu2013hybrid}, model agnostic meta learning \cite{adapting_gong_2022}, and knowledge distillation \cite{collaborative_kong_2020}. 

In replay-based methods, a certain part of previously encountered data is stored and reused in the training process, which results in less overfitting to the current distribution of data instances in the sensor stream. 
Evidence of dynamic classifier learning can be witnessed in conventional approaches \cite{lu2013hybrid}, where the architecture of the classifier changes upon encountering newer tasks. 
Meta learning aims at reusing the knowledge gained from previously performed tasks in an ensemble manner, where the model agnostic approaches, in particular, deal with using as little finetuning data as possible for the target task using the parameters learned in the previously performed tasks. 
Lastly, the knowledge distillation frameworks consist of a teacher-student pair, where the teacher model is usually a high-capacity model, which is mimicked by the student model in terms of its inference. 
Thus, the student model is trained on the incoming streaming data whereas the training is guided by the teacher model, which is already trained on a bigger data corpus. \thomas{You are using too many commas (in general). If in doubt, leave it out ...}

Another practical scenario addressed in the literature is the training across multiple decentralized devices in a federated learning setup \cite{semisupervised_presotto_2022}.
In this setup, rather than performing the training on a single device with the entire dataset, the model is trained locally in a separate manner thereby using subsets of local data available on each client side. 
Then, the model updates are shared across the network to maintain global as well as local copies. 
There have been works that target the nature of the global as well as local updates in a transfer learning setting \cite{federated_gudur_2020}. 
Since the sharing of data is not allowed \thomas{Sloppy. Rephrase.}, models, parameter updates, and confidence scores are the aspects that are shared across the server and the client \cite{semisupervised_hashemian_2021}. 

\subsection{Knowledge-Base Transfer}
\label{subsec:kb_transfer}
While classifying transfer learning approaches based on the question of \textit{what} is transferred, many prominent works \cite{pan2009survey, weiss2016survey} consider instance, feature, parameter, and relational-knowledge transfer methods. 
In the last type, i.e., relational knowledge transfer, the source and the target domains are assumed to be non-i.i.d. \thomas{?} and bound by multiple relations. 
This assumption of having relational data is not true for the datasets used in the HAR community.  \thomas{Why?}
Moreover, we observe \thomas{Nope.} methods in our literature survey that transfer knowledge snippets that are neither data instances, feature spaces, or parameters nor relational knowledge.  
Instead, they represent domain-specific metadata, heuristics, or context information, which is leveraged in the instance, feature, and parameter transfer techniques. 
Thus, in this survey, we classify such methods under knowledge-base transfer, which includes the transfer of relational as well as other types of knowledge snippets across domains. 

Under \thomas{"Under"?} the relational knowledge transfer, we observe \thomas{Nope.} cognitive science based approach using the concept of knowledge graphs \cite{anjomshoaa2021transfer}. \thomas{Rephrase.} 
First, statistical metadata with respect to the involved domains is collected followed by building a knowledge graph in a schematic representation. 
This knowledge graph is then transferred and the metadata is updated with target domain statistics to perform inference. 

The majority of knowledge-based transfer works lie in the non-relational knowledge transfer paradigm, where source domain specific metadata \cite{yu2023optimal}, heuristics \cite{rashidi2010multi}, and context information \cite{cook2010learning} are leveraged in the target domain training. 
For example, to perform feature transfer across smart home domains, sensor IDs are allocated depending on their placement in smart homes \cite{cook2010learning}.
Sensors from similar locations (like kitchen, living space, bedroom, etc.) share the same sensor ID. 
This process of assigning sensor IDs is guided using context information from the source domain. 
In another example, while selecting the most optimal \thomas{Really? Still?} source domain for a given target domain, a similarity metric is used, which depends on the commonalities between domains in terms of common sensor modalities and locations \cite{yu2023optimal}.
This is a classic example of domain metadata being transferred in knowledge-base transfer. 

There have also been works, where domain heuristics are leveraged. 
For example, in one of the foundational works of transfer learning in smart home settings \cite{rashidi2010multi}, activity templates are formed by merging similar activity labels across multiple domains. 
This requires the transfer of domain heuristics to perform the merging step. 
Such transfers are also found in self-supervised pre-training methods based on sensor \cite{autonomous_rokni_2016}, modality \cite{deep_li_2020}, and domain \cite{less_hu_2016} specific context data. 
We note that the aforesaid approaches are always used in combination of instance, feature, or parameter transfer techniques, and are rarely used standalone. 








==> data.tex <==
\textcolor{blue}{Add the quadrant figure from CISCO slides (slide no 18) and plot example works on it.} \\ \\
\textcolor{blue}{Paragraph 1: Using this figure, explain each quadrant, what it signifies, and which practical scenarios are covered in it. Describe the challenges involved in non (+,+) quadrants.}\\ \\
\textcolor{blue}{Paragraph 2: Talk about the "amounts" of data involved. Which works require more/less amounts, why do they require those quantities, what is a reasonable assumption about the data requirements in literature, etc.
Try to extract trends from existing works. Talk about useful outlier works in each quadrant (preferable works are towards the origin). How do they achieve it? } \\ 
\textcolor{blue}{Here, talk explicitly about the Data and NOT the annotations!} \\ \\
\textcolor{blue}{Paragraph 3: Transition from data to annotations availability. Analyze them using the same factors as the ones for data availability.
Finally, list down all 16 configurations of (source data, source labels, target data, target labels) under (more/less) categories. Remove impossible ones (like less source data, more source annotations, etc.) are discuss which ones are focused more vs. which ones NEED TO BE focused more.}\\ \\
\textcolor{blue}{Paragraph 4: Point out holes in literature, which of these configurations are explored in what modalities/use cases. What can be possible future directions based on this more/less and present/absent analysis?}

\thomas{Will we actually have enough material for an entire section on this?}
\thomas{Aren't sections 3 and 4 part of the background (conceptually)?}


==> modalities.tex <==

\textcolor{blue}{Paragraph 1: Describe why we want this categorization: Transfer across the same modality vs. different modalities. Both have practical applications, describe them. \\
Describe the challenges associated with same-modality transfer: For instance, same sensor type (say accelerometer) but different sensor position/location/orientation/etc. \\
Describe the challenges associated with different-modality transfer: Discuss possible transfer pairs, loss of information (say video-to-IMU), which transfers make sense, why, etc.
}
\subsection{Transfer across same modalities}
\textcolor{blue}{Each paragraph would target a modality (say accelerometer to accelerometer transfer) and list down (and explain) works under that category from a modality transfer viewpoint (for eg, don't discuss other methodology contributions, just explain how they transferred across the same modality, buy say, different sensor location/position/etc.)}

\subsection{Transfer across different modalities}
\textcolor{blue}{ First, describe 2 interpretations of heterogeneous TL in literature: multi-sensor transfer and sensor-to-sensor transfer.\\ Although sensor-to-sensor transfer is important here, other one is also does it non-explicitly.  \\
Each paragraph would target a source-target modality pair: explain the challenges involved. \\
Next, draw a graph where nodes are modality types and directed edges represent source-to-target transfers explored in literature. Comment on the aspects of loss-of-information, if any, then why would we (or they) prefer this transfer (what was the limiting factor in the source modality), and comment on the aspect of which modality is favorable/more informative/useful under what circumstances. Discuss the possibility of reverse transfer and point out missing transfer pairs in the literature. \\ \\
Include a table that lists down works and tags them as same/different modality transfer and also the actual transfer category (video-to-IMU or accelerometer-to-accelerometer)}

\begin{table}[]
\caption{Homogeneous vs. Heterogeneous TL}
\label{tab:modality_TL}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l}
\hline
                                        Classify Further\\ (IMU-to-IMU, vid-to-vid, img-to-img, etc. for same modality)\\
                                        (multi-modal heterogeneous vs. sensor-to-sensor heterogeneous \\in heterogeneous TL) & References                                                                                                 \\ \hline
Transfer across different modalities (Heterogeneous TL) & \begin{tabular}[c]{@{}l@{}}~\cite{finetuning_yu_2023},~\cite{audiovisual_zhou_2021},~\cite{collegial_feuz_2017},~\cite{crossmodal_yang_2022},~\cite{deep_ordonez_2016},~\cite{deep_li_2020},~\cite{deep_yan_2022},~\cite{deeptranshar_kumar_2023},~\cite{digging_hoelzemann_2020},~\cite{enabling_xing_2018}\\ ~\cite{enabling_medrano_2019},~\cite{heterogeneous_feuz_2014},~\cite{human_varshney_2021},~\cite{inertialvision_abebe_2017},~\cite{instilling_wei_2016},~\cite{label_sukhija_2018},~\cite{modelagnostic_alinia_2023},~\cite{stadapter_pan_2022},~\cite{supervised_sukhija_2018},~\cite{supervised_sukhija_2019}\\ ~\cite{transfer_hernandezcruz_2021},~\cite{transfer_feuz_2015},~\cite{transfer_hu_2011},~\cite{unsupervised_sanabria_2021}, ~\cite{hajifar2021investigation} (and counting)\end{tabular} \\
Transfer across same modality                           & Remaining out of pool of $\sim$233 (and counting)                                                          \\ \hline
\end{tabular}%
}
\end{table}

\thomas{Will we actually have enough material for an entire section on this?}
